Theory for identification and Inference with Synthetic Controls: A Proximal Causal Inference Framework

Synthetic control (SC) methods are commonly used to estimate the treatment effect on a single treated unit in panel data settings. An SC is a weighted average of control units built to match the treated unit, with weights typically estimated by regressing (summaries of) pre-treatment outcomes and measured covariates of the treated unit to those of the control units. However, it has been established that in the absence of a good fit, such regression estimator will generally perform poorly. In this paper, we introduce a proximal causal inference framework to formalize identification and inference for both the SC and ultimately the treatment effect on the treated, based on the observation that control units not contributing to the construction of an SC can be repurposed as proxies of latent confounders. We view the difference in the post-treatment outcomes between the treated unit and the SC as a time series, which opens the door to various time series methods for treatment effect estimation. The proposed framework can accommodate nonlinear models, which allows for binary and count outcomes that are understudied in the SC literature. We illustrate with simulation studies and an application to evaluation of the 1990 German Reunification.

==> background_en.tex <==

\usepackage{natbib}

\usepackage{amsfonts,amssymb,amsmath,amsthm}
\usepackage{color,graphicx,float,booktabs,subfig,hyperref,bm,multirow,threeparttable,textcomp}
\usepackage{tikz}
\usetikzlibrary{positioning,shapes.geometric}



\theoremstyle{plain}
\newtheorem{assumption}{\bf Assumption}
\newtheorem{condition}{\bf Condition}
\newtheorem{theorem}{\bf Theorem}
\newtheorem{result}{\bf Result}
\newtheorem{lemma}{\bf Lemma}
\newtheorem{example}{Example}
\newtheorem{definition}{Definition}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{property}{Property}
\newtheorem{remark}{Remark}



\makeatletter
\def\pr{{f}}
\def\tpr{\tilde {f}}
\def\logit{\text{logit}}
\def\expit{\text{expit}}
\def\t{{ \mathrm{\scriptscriptstyle T} }}
\def\cov{{\rm cov}}
\def\var{{\rm var}}


\def\T{{\mathcal  T}}
\def\IFfun{{\rm  IF}}
\def\EIF{{\rm  EIF}}
\def\IFset{{\mathcal{IF}}}
\def\NIF{{\rm  NIF}}
\def\eff{{\rm eff}}

\def\OR{{\rm  OR}}
\def\NP{{\rm  NP}}
\def\NDE{{\rm  NDE}}
\def\NIE{{\rm  NIE}}
\def\R{{\mathcal R}}
\def\N{{\mathcal N}}
\def\H{{\mathbb H}}
\def\dt#1{\overset{\hbox{\huge .}}{#1}}
\makeatother

\renewcommand{\thesubfigure}{\roman{subfigure}} \makeatletter


%\newcommand{\red}{\color{red}}
%\newcommand{\blue}{\color{blue}}
\definecolor{darkblue}{rgb}{0.0,0.0,0.6}
%\newcommand{\darkblue}{\color{darkblue}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\darkblue}[1]{\textcolor{darkblue}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}



\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\makeatletter
\newcommand*{\ind}{%
	\mathbin{%
		\mathpalette{\@ind}{}%
	}%
}
\newcommand*{\nind}{%
	\mathbin{% % The final symbol is a binary math operator
		\mathpalette{\@ind}{\not}% \mathpalette helps for the adaptation
	}%
}
\newcommand*{\@ind}[2]{%
	\sbox0{$#1\perp\m@th$}% box 0 contains \perp symbol
	\sbox2{$#1=$}% box 2 for the height of =
	\sbox4{$#1\vcenter{}$}% box 4 for the height of the math axis
	\rlap{\copy0}% first \perp
	\dimen@=\dimexpr\ht2-\ht4-.2pt\relax
	\kern\dimen@
	{#2}%
	\kern\dimen@
	\copy0 % second \perp
} 
\makeatother



\setlength{\oddsidemargin}{0pt}
\setlength{\evensidemargin}{0pt}
\setlength{\topmargin}{-20pt}
\setlength{\headsep}{10pt}
\setlength{\headheight}{14pt}
\addtolength{\textheight}{1.3in}
\setlength{\textwidth}{6.5in}
\setlength{\parindent}{2em}


%\linespread{2}






==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
